Simple, Interpretable and Stable Method for Detecting Words with Usage Change across Corpora

The problem of comparing two bodies of text and searching for words that differ in their usage between them arises often in digital humanities and computational social science. This is commonly approached by training word embeddings on each corpus, aligning the vector spaces, and looking for words whose cosine distance in the aligned space is large. However, these methods often require extensive filtering of the vocabulary to perform well, and - as we show in this work - result in unstable, and hence less reliable, results. We propose an alternative approach that does not use vector space alignment, and instead considers the neighbors of each word. The method is simple, interpretable and stable. We demonstrate its effectiveness in 9 different setups, considering different corpus splitting criteria (age, gender and profession of tweet authors, time of tweet) and different languages (English, French and Hebrew).

==> Makefile <==
# set latexfile to the name of the main file without the .tex
#latexfile = eacltest
latexfile = semantic_change
# put the names of figure files here.  include the .eps
figures = 

#includedfiles = Intro.tex State-of-the-art.tex Experiments.tex Discussion.tex
includedfiles = 
#Sec_7_1_Qualitative_analysis.tex Makefile table_interesting_examples.tex djame.tex











#Algos.tex Discussion.tex Results.tex \
#	eacltest.tex experiences.tex intro.tex lexical-inpact.tex \
#	presentation-treebank.tex protocol.tex state-of-the-art-comparaison.tex\
#	corpus-setup-experiment.tex TODO.tex Tagset.tex crossparsing.tex \
#	new_intro.tex new_presTB.tex new_protocol.tex examples-marie.tex

TEX = pdflatex

# *.fig files may be in ./Figs
vpath %.fig Figs


all: pdf
$(latexfile).dvi : $(figures) $(includedfiles) $(latexfile).tex


%.eps : %.fig
	fig2dev -L eps $< > $@

$(latexfile).pdf : $(latexfile).tex $(includedfiles) $(figures)
	$(TEX)  $(latexfile).tex
#	$(TEX)  appendix.tex

pdf :	$(latexfile).pdf 

bib : $(latexfile).tex
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
	 
force:
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

appendix.pdf: 
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

	

$(latexfile).ps : $(latexfile).dvi
	dvips  -Ppdf $(latexfile) -o $(latexfile).ps

ps : $(latexfile).ps 

$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig

tarball: $(latexfile).tar.gz


clean: 
	rm -f $(latexfile).bbl
	rm -f $(latexfile).log
	rm -f $(latexfile).dvi
	rm -f $(latexfile).blg
	rm -f $(latexfile).aux
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf
	rm -f $(latexfile).out
	
clean2:
	rm -f appendix.bbl
	rm -f appendix.log
	rm -f appendix.dvi
	rm -f appendix.blg
	rm -f appendix.aux
	rm -f appendix.ps
	rm -f appendix.pdf
		
check:
	cat $(latexfile).log | grep --text undef

dist-clean: clean
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf

viewX: pdf 
	open $(latexfile).pdf
	
viewA: pdf
	open -a Preview.app $(latexfile).pdf

view: pdf
	open -a Skim.app $(latexfile).pdf
#	open -a Skim.app appendix.pdf 

gv: ps
	gv $(latexfile).pdf


edit: 
	xemacs $(latexfile).tex &


up:
	git pull

co:	commit
	
commit:
	git commit -m "update djame" 	./
	git push

commitsvn:
	svn commit -m "update" ./

upsvn:
	svn up



ebib:
	open emnlp2014.bib
	

==> table_interesting_examples.tex <==
\pdfoutput=1 
\begin{table*}[h!]
%\resizebox{1\linewitdh}{!}{% resizebox
%\begin{adjustbox}{max width=0.77\textwidth}
\begin{center}
{\footnotesize
\begin{tabular}{llL{0.4\linewidth}}
\hline
  {\sc Splits}& {\sc Top 10} & {\sc Context} \\
\hline
{\bf English} & van & captain vs vehicule \\
{\bf (diachronic. 90y)} & press & printing vs places \\
 & oxford & location vs University \\
\midrule
{\bf Age} & dem & them vs the political party \\
{\bf (young vs older)} & dam & damn vs water barrier \\
 & assist & football contribution vs help \\
\midrule
{\bf Gender} & clutch & grasping vs female bag) \\
{\bf (male vs female)} & bra & variation of {\em bro} vs. underwear \\
 & gp & grand prix event  vs. general practitioner \\
\midrule
{\bf Occupation} & cc & carbon copy vs. country club \\
{\bf (Performer vs Sport)} & duo & duet vs. pair of people \\
 & wing & politics vs. football player position \\
\midrule
{\bf Occupation} & op & event opening vs operation \\
{\bf (Creator vs Sport)} & wing & politics vs. football player position \\
 & worlds & earth vs world cup \\
\midrule
{\bf Time of week} & cc & credit card vs carbon copy \\
{\bf (weekday vs week-end)} & pitch & presentation attribute vs. playing surface \\
 & bond & agreement vs.  fictional character \\
\midrule
{\bf French diachronic. 4y} & ia & variant of ya/there is vs Fr. AI acronym  \\
{\bf (2014 vs 2018)} & divergent & the movie vs the adjective \\
\midrule
{\bf Hebrew diachronic. 4y} & beelohim-in god & pledge word vs. religion-related \\
{\bf ( ???? Vs ????)} & Kim-Kim & First name vs. Kim Jong-un \\
\hline
\end{tabular}
\caption{Interesting \hl{usage?/semantic?} changes found at the top 10
 ranks  by our method for each split }
\label{tab:exemple:interesting_usage:top10}
}%eof foot
\end{center}
%}% resizebox
%\end{adjustbox}
\end{table*}


\begin{table*}[h!]
%\resizebox{1\linewitdh}{!}{% resizebox
%\begin{adjustbox}{max width=0.77\textwidth}
\begin{center}
{\footnotesize
\begin{tabular}{llL{0.4\linewidth}}
\hline
  {\sc Splits}& {\sc Top 10} & {\sc Context} \\
\hline
{\bf English} & headed & body part vs move to a direction \\
{\bf (diachronic. 90y)} & mystery & difficulty in understanding smthg vs litterature genre \\ 
\midrule 
{\bf Age} & pc & computer vs Canadian Political Party \\
{\bf (young vs older)} & presents & noun vs verb \\
 & wing & general vs political meaning \\
\midrule 
{\bf Gender} & stat & (statistics vs. right away) \\
{\bf (male vs female)} & pit & car-related vs. dog-related \\
 & dash & radio station vs. quantity \\
\midrule 
{\bf Occupation} & jazz & music genre vs. basket- ball team \\
{\bf (Performer vs Sport)} & stages & platforms vs. company(bikes) \\
 & record & music record vs. achievement \\
\midrule 
{\bf Occupation} & oval & oval office vs. sports ground \\
{\bf (Creatorr vs Sport)} & fantasy (?) & genre vs. fantasy football \\
 & chilling & frightening vs. relaxing \\
\midrule 
{\bf Time of week} & Sunday & weekday vs vacation-related \\
{\bf (weekday vs week-end)} & vp & vice-president vs tv-series* \\
 & fight & general meaning vs boxing \\
\midrule 
{\bf French diachronic. 4y} & pls & contraction of Eng ``please'' vs the acronym for lateral safety position \\
{\bf (2014 vs 2018)} & apl & contraction of appeler/to call vs apl, controversial housing subsidies \\
\midrule 
{\bf Hebrew diachronic. 4y} & shtifat~washing & plumbing vs. brain- washing \\ 
{\bf ( ???? Vs ????)} & miklat~shelter & building vs. asylum (for
refugees) \\ 
\hline
\end{tabular}
\caption{Interesting \hl{usage?/semantic?} changes found at the top 30
 ranks  by our method for each split }
\label{tab:exemple:interesting_usage:top10}
}%eof foot
\end{center}
%}% resizebox
%\end{adjustbox}
\end{table*}




